Computing over Data Streams using Catalytic Space

We introduce a streaming model with \emph{catalytic memory}, an auxiliary workspace that must be returned to its initial state at the end of the computation. We show that catalytic space yields dramatic space savings for data stream algorithms. We first study the exact computation of frequency moments in insertion-only data streams. For every $k\ge1$, we give an exact four-pass algorithm for computing $\mathbb{F}_{k}$ using $O(k\log m)$ clean space, where $m$ is the stream length. We also present a $(k+1)$-pass algorithm with the same clean-space complexity that uses a factor of $k$ less catalytic space than the four-pass algorithm. For small moments, we obtain stronger results. In particular, we show that $\mathbb{F}_{2}$ and $\mathbb{F}_{3}$ can be computed exactly in two and three passes, respectively, using only $O(\log m)$ clean space. Additionally, we show that exact $\mathbb{F}_{0}$ computation reduces to computing $\mathbb{F}_{k}$ for a suitably chosen large value of $k$, resulting in an exact four-pass algorithm for $\mathbb{F}_{0}$ using only $O(\log m)$ clean space. We further show how our frequency-moment algorithms can be used to exactly count induced occurrences of any fixed graph $H$ in a graph stream, yielding a four-pass algorithm that uses $O_H(\log n)$ clean space, where $n$ is the number of vertices in the graph. As a special case, we obtain an exact three-pass algorithm for triangle counting using $O(\log n)$ clean space. All of our algorithms are multi-pass. We complement these algorithmic results with a matching limitation showing that catalytic memory does not provide additional power in the single-pass setting. Specifically, we prove that every randomized or deterministic single-pass streaming algorithm using $s$ bits of clean memory and catalytic space can be simulated in the standard streaming model, without catalytic memory, using $O(s)$ space.

==> Sections/F3in3-old.tex <==

\subsubsection{$F_3$ in 3 pass}

Let us now try for a $3$-pass algorithm for $f_3$. We again do a similar breakdown, and consider $\ffreqvec$ and $\bfreqvec$. In this case, we have:
\[
\sum_{i} \freqvec_i^3 = \sum_i \fbrac{\ffreqvec_i^3+\bfreqvec_i^3} = \sum_i \ffreqvec_i^3 + \sum_i \bfreqvec_i^3 + 3 \sum_i \ffreqvec_i^2\bfreqvec_i + 3 \sum_i \ffreqvec_i\bfreqvec_i^2
\]

Now, we want to compute $\sum_i \ffreqvec_i^2\bfreqvec_i$, and $\sum_i \ffreqvec_i\bfreqvec_i^2$. 

\begin{algorithm}
    \caption{$f_3$-Recursion Step}
    \begin{algorithmic}
        \Require $\streamlen \gets $length of the stream, Catalytic spaces $\cat$, $\cattwo$, $\catthree$, $\catfour$
        \State \textbf{Pass $0.5$}
        \State $U  = 0$
        \State $S = 0$
        \For{each element $u$}
            \State $U = U + \cattwo[i]$
            \State $\cat[i] \gets \cat[i]+1$
            \State $S = S + \catthree[i]^2$
            \State $\catfour[i] \gets \catfour[i]+ \catthree[i]$ \Comment{Additional Step for $f_3$}
        \EndFor
        \State \textbf{Final States:} \red{$\cat[i] = \cat_i +\ffreqvec_i$, $\catfour[i] = \catfour_i + \catthree_i\ffreqvec_i$}\\
        \red{$U = \sum_i \cattwo_i\ffreqvec_i$, $S = \sum_i \catthree_i^2\ffreqvec_i$} 
        \State \textbf{Pass $1$}
        \State Initialize $X = 0$
        \For{each element $u$}
            \State $X = X + \cat[u]^2$ \Comment{Modified for $f_3$}
            \State $Y = y + \catfour[u]$\Comment{Additional Step for $f_3$}
            \State $\catthree[u] = \catthree[u] + 1$\Comment{Additional Step for $f_3$}
        \EndFor
        \State \textbf{Final States:} \red{$\catthree[i] = \catthree_i+\bfreqvec_i$}, \blue{$\cat[i] = \cat_i +\ffreqvec_i$, $\catfour[i] = \catfour_i + \catthree_i\ffreqvec_i$}\\
        \red{$X = \sum_i \fbrac{\cat_i+\ffreqvec_i}^2\bfreqvec_i$, $Y = \sum_i \fbrac{\catfour_i+\catthree_i\ffreqvec_i}\bfreqvec_i$}, $U = \sum_i \cattwo_i\ffreqvec_i$, $S = \sum_i \catthree_i^2\ffreqvec_i$
        \State \textbf{Pass $1.5$}
        \State Initialize $Z = 0$
        \For{each element $u$}
            \State $\cat[u] = \cat[u]-1$
            \State $Z = Z + \catthree[u]^2$
        \EndFor
        \State \textbf{Final States:} \green{$\cat[i] = \cat_i$} , \blue{$\catthree[i] = \catthree_i+\bfreqvec_i$, $\catfour[i] = \catfour_i + \catthree_i\ffreqvec_i$}\\
        \red{$Z = \sum_{i}(\catthree_i+\bfreqvec_i)^2\ffreqvec_i$}, $X = \sum_i \fbrac{\cat_i+\ffreqvec_i}^2\bfreqvec$, $Y = \sum_i \fbrac{\catfour_i+\catthree_i\ffreqvec_i}\bfreqvec_i$, $U = \sum_i \cattwo_i\ffreqvec_i$, $S = \sum_i \catthree_i^2\ffreqvec_i$
        \State \textbf{Pass 2}
        \State Initialize $W = 0$
        \For{each element $u$}
            \State $\cattwo[u] = \cattwo[u] + \cat[u]$
            \State $W = W + \cat[w]^2$
            \State $\catthree[u] = \catthree[u]-1$
        \EndFor
        \State \textbf{Final States: } \red{$\cattwo[i] = \cattwo_i+\cat_i\bfreqvec_i$}, \green{$\catthree[i] = \catthree_i$}, \blue{ $\catfour[i] = \catfour_i + \catthree_i\ffreqvec_i$}\\
        \red{$W = \sum_i \cat_i^2\bfreqvec_i$}, $Z = \sum_{i}(\catthree_i+\bfreqvec_i)^2\ffreqvec_i$, $X = \sum_i \fbrac{\cat_i+\ffreqvec_i}^2\bfreqvec$, $Y = \sum_i \fbrac{\catfour_i+\catthree_i\ffreqvec_i}\bfreqvec_i$, $U = \sum_i \cattwo_i\ffreqvec_i$, $S = \sum_i \catthree_i^2\ffreqvec_i$
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
    \caption{$f_3$-Recursion Step - Continued}
    \begin{algorithmic}
        \Require $\streamlen \gets $length of the stream, Catalytic spaces $\cat$, $\cattwo$, $\catthree$, $\catfour$
        \State \textbf{Pass 2.5}
        \State $T = 0$
        \For{ each element $u$}
            \State $\catfour[i] = \catfour[i] - \catthree[i]$
            \State $T = T + \cattwo[i]$
        \EndFor
        \State \textbf{Final States: } \blue{$\cattwo[i] = \cattwo_i+\cat_i\bfreqvec_i$}, \green{$\catfour[i] = \catfour_i$}\\
        \red{$T = \sum_i \fbrac{\cattwo_i+\cat_i\bfreqvec_i}\ffreqvec_i$}, $W = \sum_i \cat_i^2\bfreqvec_i$, $Z = \sum_{i}(\catthree_i+\bfreqvec_i)^2\ffreqvec_i$, $X = \sum_i \fbrac{\cat_i+\ffreqvec_i}^2\bfreqvec$, $Y = \sum_i \fbrac{\catfour_i+\catthree_i\ffreqvec_i}\bfreqvec_i$, $U = \sum_i \cattwo_i\ffreqvec_i$, $S = \sum_i \catthree_i^2\ffreqvec_i$
        \State \textbf{Pass $3$:}
        \State Initialize $V = 0$
        \For{each element $u$}
            \State $\cattwo[u] = \cattwo[u]-\cat[u]$
            \State $V = V + \catfour[u]$
        \EndFor
        \State \textbf{Final States: } \green{$\cattwo[i] = \cattwo_i$}\\
        \red{$V = \sum_i \catfour_i\bfreqvec_i$}, $T = \sum_i \fbrac{\cattwo_i+\cat_i\bfreqvec_i}\ffreqvec_i$, $W = \sum_i \cat_i^2\bfreqvec_i$, $Z = \sum_{i}(\catthree_i+\bfreqvec_i)^2\ffreqvec_i$,\\ $X = \sum_i \fbrac{\cat_i+\ffreqvec_i}^2\bfreqvec$, $Y = \sum_i \fbrac{\catfour_i+\catthree_i\ffreqvec_i}\bfreqvec_i$, $U = \sum_i \cattwo_i\ffreqvec_i$, $S = \sum_i \catthree_i^2\ffreqvec_i$
        \State \textbf{Postprocessing: }
        \State $\sum_i \ffreqvec_i^2\bfreqvec_i =  X - W - 2(T-U)$
        \State $\sum_i \ffreqvec_i\bfreqvec_i^2 = Z - S - 2(Y-V)$
    \end{algorithmic}
\end{algorithm}



==> Sections/Fkinkpassalgo.tex <==


\subsubsection{Algorithm}

The algorithm to compute $\FM{k}(\stream)$ for any $k \geq 2$, with $k+1$ passes is described in Algorithm~\ref{alg:FkinKP+1}. The algorithms uses $n$ catalytic registers  $\C{C}[i]$ for $i\in [n]$ where each $\C{C}[i]$ can hold $\log M = \lceil k\log_2 mk\rceil$ bits.  

%{\color{red} We need to mention: (1) Adverserial Pass Algorithms (2) This Algorithm can be modified to computes all $\FM{k}$ in $k+1$ passes.}

% \begin{algorithm}
% \caption{Stream Power Sum Algorithm}
% \label{alg:FkinKPlus1}
% \begin{algorithmic}[1]
% \Require stream $\texttt{A}$, array $\texttt{C}$ of size $n$, integers $n, k$

% \State $\texttt{sum} \gets 0$

% \For{$j \gets 0$ to $k$}
%     \For{$i \gets 0$ to $n-1$}
%         \State $\texttt{sum} \gets \texttt{sum} + (-1)^j \binom{k}{j} \cdot (\C{C}[i])^k$
%     \EndFor
    
%     \If{$j = k$}
%         \For{each $a$ in $\texttt{A}$}
%             \State $\C{C}[a] \gets \C{C}[a] - k$
%         \EndFor
%     \Else
%         \For{each $a$ in $\texttt{A}$}
%             \State $\C{C}[a] \gets \C{C}[a] + 1$
%         \EndFor
%     \EndIf
% \EndFor

% \State $\texttt{sum} \gets \dfrac{\texttt{sum}}{k! \cdot (-1)^k}$

% \State \Return $\texttt{sum}$

% \end{algorithmic}
% \end{algorithm}

%\violet{Debarshi: Does taking$\mod M$ only in line 5 suffice? Maybe we should add $M$ to $\texttt{sum}$ every time the modulo operation happens.}

\begin{algorithm}
\caption{Stream Power Sum Algorithm}
\label{malg:FkinKP+1}
\begin{algorithmic}[1]
\Require stream $\stream = \langle x_1, \dots, x_{\streamlen}\rangle$, catalytic space $\C{C}$ 


\State $M \gets 2^{\lceil\log \streamlen^kk!+1\rceil}$
\State $\texttt{sum} \gets (-1)^k\sum_i  (\C{C}[i])^k \mod M$ \Comment{\color{blue} \texttt{sum} =  $(-1)^k\sum_i (\cc{c}[i])^k$} \color{black}

\ 

\For{\textbf{Pass}\ \ $j \gets 1$ to $k$} 

\ 

  \For{$ i \gets 1$ to $\streamlen$}    
       \State $\C{C}[x_i] \gets (\C{C}[x_i] +  1) \mod M$ \Comment{\color{blue} $\C{C}[i] = \cc{c}[i] + j\f_i$} \color{black}
  \EndFor



 \State $\texttt{sum} \gets \texttt{sum} + \sum_i (-1)^{j+k} \binom{k}{j} \cdot (\C{C}[i])^k \mod M$ 
 \
 
 \Comment{\color{blue} \texttt{sum} =  $\sum_i \sum_{\ell = 0}^j(-1)^{\ell+k} \binom{k}{\ell} \cdot (\cc{c}[i] + \ell\f_i)^k$}\color{black}
\EndFor

%\State $\texttt{sum} \gets \dfrac{\texttt{sum}}{k! \cdot (-1)^k}$

 

\textbf{/* Pass $(k+1)$ */}

\ 

\For{$ i \gets 1$ to $\streamlen$}    
        \State $\C{C}[x_i] \gets (\C{C}[x_i] - k) \mod M$ \Comment{\color{blue}{$\C{C}[i] = \cc{c}[i]$}}\color{black}
\EndFor

\ 

\State \Return $\frac{\texttt{sum}}{k!}$ %\sum_i (-1)^j \binom{k}{j} \cdot (\C{C}[i])^k$


%\State \Return $\texttt{sum}$

\end{algorithmic}
\end{algorithm}

The following claim, which is easy to see, captures the basic behaviour of the algorithm. 

\begin{claim}\label{mClaim: FkinK+1 States}
    For any $j \leq k$, at the end of the $j$-th pass, the catalytic space contains
    \[
    \C{C}[i] =( \cc{c}[i] + j\f_{i}) \mod M
    \]
    At the end of the $k+1$-th pass, the catalytic space contains
    \[
    \C{C}[i] = \cc{c}[i] 
    \]
    Furthermore, at the end of $j$-th pass for any $j \leq k$, the counter $\texttt{sum}$ contains 
    \[
    \texttt{sum} =  \sum_i \sum_{\ell = 0}^j(-1)^{\ell+k} \binom{k}{\ell} \cdot ((\cc{c}[i] + \ell\f_i) \mod M)^k \mod M
    \]
\end{claim}

%{\color{red} Why are we writing as $l-k$ in the exponent? $l \leq k$ so $k-l$ makes more sense. Also, I am not quite sure ${\tt sum}+n$ coming in the expression in the algorithm. Cant we fold it into the sum?} \violet{Fixed?}

Proof of the following lemma is presented later.
\begin{lemma}\label{mLem: Freq Moment Binomial Identity}
    For any $\cc{c}$ and $\f$, and $k \in \Nat$, we have 
    \[
        \sum_{j=0}^{k}(-1)^j\binom{k}{j}(\cc{c}+j\f)^k = \f^k(-1)^kk!
    \]
\end{lemma}
   

    \begin{corollary}\label{mcoro:identity}
       For any $i\in [n]$,  $\sum_{\ell = 0}^j (-1)^{\ell+k} \binom{k}{\ell} \cdot ((\cc{c}[i] + \ell\f_i) \mod M)^k = ((\f_i)^kk!) \mod M$
    \end{corollary}

    % \begin{proof}
    %     The 
    % \end{proof}

\begin{theorem}\label{mthm:kplus1}
    \Cref{malg:FkinKP+1} takes as input a stream $\stream$ uses $k+1$ passes, $\bigo{k\log \streamlen k}$ clean space and $\bigo{n}$ catalytic space and outputs the value of $\FM{k}(\stream)$.
    
    %makes $k+1$ passes, uses \red{$\bigo{k\log m}$} space returns $\norm{\f}_k^k$.
\end{theorem}

\begin{proof}
    By \Cref{mClaim: FkinK+1 States}, we have that at the end of the $k$-th pass,
    % \[
    % \texttt{sum} =  \sum_{\ell = 0}^k\sum_i (-1)^{\ell+k} \binom{k}{\ell} \cdot (\cc{c}[i] + \ell\f_i)^k
    % \]
    % Then, we have {\color{red} Is the following true? Where does the $n$ come from? Shouldn't the $\ell = 0$ term be $\sum_i(-1)^k(\cc{c}[i])^k$, not $n$}
    \begin{align*}
        \texttt{sum} = &(\sum_i \sum_{\ell = 0}^k (-1)^{\ell+k} \binom{k}{\ell} \cdot ((\cc{c}[i] + \ell\f_i)\mod M)^k) \mod M&\\
        = & \left(\sum_{i} \f_i^kk!\right)\mod M & \mbox{[From Corollary~\ref{mcoro:identity}]}\\
        = & k!\sum_{i} \f_i^k & \mbox{[Since $M \geq k!\sum_{i} \f_i^k$.]}
    \end{align*}
    Hence, we have $\frac{\texttt{sum}}{k!} = \sum_i \f_i^k = \FM{k}(\stream)$, which the algorithm returns. Note that the only non-catalytic space that is needed is to store the variables $\texttt{sum}$, $i$, and $j$. Note that the maximum value  $\texttt{sum}$ can take is $M$, leading to a space bound of $O(k \log mk)$.
\end{proof}

\vspace{2mm}    
\noindent{\em Remark:} The \(k+1\)-pass algorithm is stronger than a standard multi-pass streaming algorithm in the following sense. In the traditional multi-pass model, every pass sees the stream in the same order. In contrast, the algorithm for \(\FM{k}\) works even if, on each pass, an adversary presents the elements in an arbitrary order, as long as the underlying stream itself is unchanged.

